DriveVLM: The Convergence of Autonomous Driving and Large Vision-Language Models

A primary hurdle of autonomous driving in urban environments is understanding complex and long-tail scenarios, such as challenging road conditions and delicate human behaviors. We introduce DriveVLM, an autonomous driving system leveraging Vision-Language Models (VLMs) for enhanced scene understanding and planning capabilities. DriveVLM integrates a unique combination of reasoning modules for scene description, scene analysis, and hierarchical planning. Furthermore, recognizing the limitations of VLMs in spatial reasoning and heavy computational requirements, we propose DriveVLM-Dual, a hybrid system that synergizes the strengths of DriveVLM with the traditional autonomous driving pipeline. Experiments on both the nuScenes dataset and our SUP-AD dataset demonstrate the efficacy of DriveVLM and DriveVLM-Dual in handling complex and unpredictable driving conditions. Finally, we deploy the DriveVLM-Dual on a production vehicle, verifying it is effective in real-world autonomous driving environments.

==> arxiv_sections/dataset.tex <==
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.75\linewidth]{imgs/scenario_type_stat.png}
%     \vspace{-1em}
%     \caption{Distribution of the scenario category in our proposed scene understanding dataset.}
%     \label{fig:scenario-type-stat}
% \end{figure*}

\vspace{-4pt}
\section{Task and Dataset}
\label{sec:dataset} 
\vspace{-2pt}
To fully exploit the potential of DriveVLM and DriveVLM-Dual in handling complex and long-tail driving scenarios, we formally define a task called \textit{Scene Understanding for Planning} (Section~\ref{sec:task-def}), together with a set of evaluation metrics (Section~\ref{sec:eval-metrics}). Furthermore, we propose a data mining and annotation protocol to curate a scene understanding and planning dataset (Section~\ref{sec:data-mining}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/data-example.pdf}
    \caption{\textbf{An annotated sample of the SUP-AD dataset.}}
    \label{fig:anno-sample}
\vspace{-0.5em}
\end{figure*}


\subsection{Task Definition}
\label{sec:task-def}
The input of Scene Understanding for Planning task comprises multi-view videos $\mathcal{V}$ from surrounding cameras and optionally 3D perception results $\mathcal{P}$ from a perception module. And its output includes the following components: \textbf{Scene Description $s$}: Composed of different conditions, object-level analysis and scene-level summary; \textbf{Meta Actions $A$}: A sequence of actions representing task-level maneuvers; \textbf{Decision Description $D$}: A detailed account of the driving decisions; \textbf{Trajectory Waypoints $W$}: The waypoints outlining the planned trajectory of the ego vehicle.
% \begin{itemize}[itemsep=0pt, leftmargin=*]
%     \item \textbf{Scene Description $s$}: Composed of different conditions, object-level analysis and scene-level summary.
%     \item \textbf{Meta Actions $A$}: A sequence of actions representing task-level maneuvers.
%     \item \textbf{Decision Description $D$}: A detailed account of the driving decisions.
%     \item \textbf{Trajectory Waypoints $W$}: The waypoints outlining the planned trajectory of the ego vehicle.
% \end{itemize}

\vspace{-0.5em}
\subsection{Evaluation Metrics}
\vspace{-0.4em}
\label{sec:eval-metrics}
To comprehensively evaluate a model's performance, we care about its interpretation of the driving scene and the decisions made. Therefore, our evaluation has two aspects: scene description/analysis evaluation and meta-action evaluation.
In the \textbf{Scene description/analysis evaluation}, we leverage a structured evaluation approach by prompting the GPT-4 to extract individual pieces of information from each scene description. Subsequently, we ask the GPT-4 to score and aggregate the results based on the matching status of each extracted piece of information. For \textbf{Meta-action evaluation}, we focus on the sequence of decision-making actions defined as meta-actions, comparing these sequences generated by the model against a ground truth using dynamic programming. To ensure the robustness of our evaluation, we use GPT-4 to generate semantically equivalent alternatives to the ground truth, with the highest similarity score determining the final decision-making accuracy. Further details on these metrics are elaborated in Appendix \textcolor{red}{B}.



% \noindent\textbf{Scene Description/Analysis Evaluation.}
% Given the subjective nature of human evaluation in scene description, we adopt a structured approach using a pre-trained LLM. This method entails comparing the generated scene description with a human-annotated ground truth description. The ground truth description encompasses structured data such as environmental conditions, navigation, lane information, and critical events with specific objects, verbs, and their influences. The LLM assesses and scores the generated descriptions based on their consistency with the ground truth.

% \noindent\textbf{Meta-action Evaluation.}
% Meta-actions are a predefined set of decision-making options. A driving decision is formulated as a sequence of meta-actions. Our evaluation method employs a dynamic programming algorithm to compare the model-generated sequences with a manually annotated ground truth sequence. The evaluation should also weigh the relative importance of various meta-actions, designating some as `conservative actions' with a lower impact on the sequence's overall context. To increase robustness, we first use the LLM to generate semantically equivalent alternatives to the ground truth sequence to enhance robustness. The sequence with the highest similarity to these alternatives calculates the final driving decision score. More details of the proposed metric are available in the Appendix \textcolor{red}{B}.

 
\subsection{Dataset Construction}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{imgs/dataset-pipeline.pdf}
    \caption{\textbf{The proposed data mining and annotation pipeline for constructing the scene understanding and planning dataset.} Scenario examples randomly sampled from the dataset (below) demonstrate the diversity and complexity of the dataset.}
    \label{fig:dataset_pipeline}
\vspace{-1em}
\end{figure*}



\label{sec:data-mining}
We propose a comprehensive data mining and annotation pipeline, shown in Figure~\ref{fig:dataset_pipeline}, to construct a \textit{Scene Understanding for Planning (SUP-AD) Dataset} for the proposed task. 
This process begins with \textbf{long-tail object mining} and \textbf{challenging scenario mining} from a large database to collect special objects and scenes like weird-shaped vehicles and road debris. For each scene, \textbf{Keyframe selection} is performed to identify crucial moments for decision-making, which are then annotated using a specialized \textbf{Scene Annotation} tool. Details of the construction process and dataset statistics are available in the Appendix~\textcolor{red}{A}.


% \noindent\textbf{Long-tail Object Mining.}
% According to real-world road object distribution, we first define a list of long-tail object categories, such as weird-shaped vehicles, road debris, and animals crossing the road. Next, we mine these long-tail scenarios using a CLIP-based search engine, capable of mining driving data using language queries from a large collection of logs. Following that, we perform a manual inspection to filter out scenes inconsistent with the specified categories.

% \noindent\textbf{Challenging Scenario Mining.}
% In addition to long-tail objects, we are also interested in challenging driving scenarios, where the driving strategy of the ego vehicle needs to be adapted according to the changing driving conditions. These scenarios are mined according to the variance of the recorded driving maneuvers.
% % Our dataset predominantly includes these challenging scenarios while incorporating a subset of non-challenging scenarios to ensure a comprehensive dataset.

% \noindent\textbf{Keyframe Selection.}
% Each scene is a video clip, it is essential to identify the `keyframe' to annotate. In most challenging scenarios, a keyframe is the moment before a significant change in speed or direction is required. We select this keyframe 0.5s to 1s earlier than the actual maneuver, based on comprehensive testing, to guarantee an optimal reaction time for decision-making. For scenes that do not involve changes in driving behavior, we select a frame that is relevant to the current driving scenario as the keyframe.

% \noindent\textbf{Scene Annotation.}
% We employ a group of annotators to perform the scene annotation, including scene description, scene analysis, and planning, except for waypoints, which can be auto-labeled from the vehicle's IMU recordings.
% To facilitate scene annotation, we make a video annotation tool with the following features: (1) the annotators can slide the progress bar back and forth to replay any part of a video; (2) while annotating a keyframe, the annotator can draw bounding boxes on the image together with language descriptions; (3) annotators can select from a list of action and decision candidates while annotating driving plans.
% Each annotation is meticulously verified by 3 annotators for accuracy and consistency, ensuring a reliable dataset for model training. Figure~\ref{fig:anno-sample} illustrates a sample scenario with detailed annotations.
% \vspace{-1em}




% \subsection{Dataset Statistics}
% The dataset comprises 1,000 scenes, each categorized into one of over 40 long-tail scenario categories. Every scene spans approximately 15 seconds and is captured using images from 6 cameras, collectively providing a 360° horizontal field of view (FOV).

% \noindent\textbf{Long-tail scenario statistics.}
% Our dataset offers a diverse array of long-tail scenarios, significantly more varied than those typically found in existing datasets. These include complex situations such as encounters with special-shaped vehicles, road debris, and animals crossing the road. The distribution of these scenario categories is depicted in Figure~\ref{fig:scenario-type-stat}. Some categories, like fallen trees on the road, are exceedingly rare, making them challenging to source in large numbers. Conversely, scenarios such as cattle on the road, while scarcely represented in most autonomous driving datasets, are abundant in our in-house databank.

% \noindent\textbf{Challenging scenario statistics.}
% Challenging scenarios are defined as those necessitating a change in the ego vehicle's driving strategy. In our dataset, these changes in strategy are quantified using meta-action sequences. We categorize meta-actions into 17 distinct types, resulting in a repertoire of over 100 unique meta-action sequences.




==> arxiv_sections/evaluation.tex <==
\section{Evaluation}
The proficiency of an autonomous driving system in accurately interpreting driving scenes and making logical, suitable decisions is of paramount importance. The evaluation approach for the Vision-Language Model (VLM) in autonomous driving, as presented in this paper, concentrates on two primary components: the evaluation of scene description and the evaluation of driving decision.
\subsection{Scene Description Evaluation}
In the context of scene description evaluation, the process of interpreting and articulating driving scenes is subject to inherent subjectivity, as there are numerous legitimate ways to express these descriptions textually. This variety makes human evaluation less feasible. 
\xiaoyu{rewrite this paragraph}
To overcome this challenge, we have devised a structured methodology for generating definitive scene descriptions. Additionally, we have integrated a Large Language Model (LLM) to assist in extracting crucial information from both the model-generated descriptions and the predefined ground truth. Following this, the same LLM is utilized to perform an assessment, which is based on the level of correspondence between the sets of information extracted.

% \includegraphics[width=0.99\columnwidth]{imgs/SceneDescription.png}

The driving scene descriptions have been methodically organized to facilitate the extraction of key information. The ground truth for scene descriptions encompasses both environmental condition description and critical event information. Environmental condition description includes weather condition, time condition, road environment, and lane condition. critical event information is a summary of the characteristics and influence of critical objects. 
We employ GPT-4 to independently extract discrete key pieces of information from both the model output and the ground truth scene descriptions. These extracted data points are then compared and quantified. Each instance of matched information is assigned a score, which is calibrated based on the extent of the match, whether complete, partial, or absent. Instances of hallucinated information incur a penalty, detracting from the overall score. The aggregate of these scores constitutes the scene description score.
\begin{align}
\begin{split}
score_{description} = \frac{1.0 \times n_{\text{matched}} + 0.5 \times n_{\text{partial}}}{n_{\text{gt}}} \\
- \frac{0.25 \times n_{\text{hallucination}}}{n_{\text{gt}}}
\end{split}
\end{align}


% \begin{align}
% score_{description} &= \frac{1.0 \times n_{matched} \nonumber \\
% &\quad + 0.5 \times n_{partial} \nonumber \\
% &\quad - 0.25 \times n_{hallucination}}{n_{gt}}
% \end{align}


The prompt for GPT-4 in evaluating scene descriptions is carefully designed, as shown in Table~\ref{}. Initially, a role prompt is employed to establish as an intelligent and logical evaluator, possessing a comprehensive understanding of appropriate driving styles. This is followed by specifying the input format, which informs GPT-4 that its task involves comparing an output description with a referenced ground truth description. This comparison is based on the extraction and analysis of key information from both descriptions, a process clearly delineated within the prompt itself. Lastly, the prompt outlines the criteria for scoring, as well as the format for the evaluation output, ensuring a structured and systematic approach to the assessment process.
\begin{table*}
\begin{tabular}{p{\textwidth}}
\toprule
% \bottomrule
% \end{tabular}
% Output Description: 
% "There is a vehicle driving in the distance in front of you, there are traffic police on the left and right, and the traffic police signal to stop."
% Reference Description: 
% "You are driving on overhead road, the navigation information telling you to go straight through this road. There are currently ego lane and left lane ahead. The right lane is an merging lane and currently separated, so you cannot change lanes to the right.  There is police officers ahead inspecting passing vehicles. The police officer in front of your lane is signaling you to stop for inspection. There are also vehicles queuing in the left lane. Based on the current driving scenario, provide subsequent reasonable driving decisions."
\textbf{System Prompt:} \\
You are a smart and logical evaluator with good knowledge of correct driving style, you will try your best to give reasonable and logical evaluation result. \\
\midrule
\textbf{Input Prompt:} \\
Given two driving scenario descriptions, one is a reference description, the other is the output description from a model, please extract key information the reference description contains and use it as comparison standards to compare how close the output descriptions is to the reference descriptions also consider each information\'s completeness. Key information extracted can be classified into environmental conditions and critical events information. environmental conditions information includes weather, time, road environment, and lane condition. Critical events information describe event related to ego vehicle\'s driving decisions, they is usually given in the format of critical object + verb/adj + influence on ego vehicle. An example of critical events information is like this: a construction zone is blocking the ego lane and the right lane in front, so the car needs to go around to avoid it. Now I will give you the reference description and the output description. \\
The reference description: \\
Weather: Sunny. || Time: Day. || Road Environment: Urban. || Lane Options: Left Lane, Own Lane, Right Lane. || Ego Lane Position: Middle Lane. \\
Critical Events: There is police officers ahead inspecting passing vehicles. The police officer in front of your lane is signaling you to stop for inspection. There are also vehicles queuing in the left lane. The right lane is an merging lane and currently separated, so you cannot change lanes to the right. \\
The output description: \\
Weather: Sunny. || Time: Day. \\
There is a vehicle driving in the distance in front of you, there are traffic police on the left and right, and the traffic police signal to stop. \\
Compare the two descriptions using extracted key information and output a similarities score on the scale from 0 to 1.0 and a explanation to describe the logic to calculate the similarity score. Each matched key information scores 1.0, and each partially matched key information score 0.5. Hallucination will also be punished, each key information exists in output but not in reference will score -0.25, the final score will be the total score divided by the number of key information extracted in the reference description. For example if total score is 1.5, and total number of key information in reference description is 3, then the final score is 1.5/3 = 0.5. Please output the detailed extraction and evaluation process. \\
\midrule
\textbf{Response:} \\
Reference description key information: \\
1. Weather: Sunny (environmental conditions)  \\
2. Time: Day (environmental conditions)  \\
3. Road Environment: Urban (environmental conditions)  \\
4. Lane Options: Left Lane, Own Lane, Right Lane (environmental conditions)  \\
5. Ego Lane Position: Middle Lane (environmental conditions)  \\
6. Police officers ahead inspecting vehicles (critical event information) \\
7. The police officer in front of ego vehicle signalling to stop (critical event information) \\
8. Vehicles queuing in the left lane (critical event information) \\
9. Cannot change to the right lane as it\'s an merging lane and currently separated (critical event information) \\
Output description key information: \\
1. Weather: Sunny. \\
2. Time: Day. \\
3. Vehicle driving in the distance in front of driver \\
4. Traffic police on the left and right \\
5. Traffic police signal to stop \\
By comparing the output to the reference: \\
- Key information 1, 2, 6, and 7 are matched, each for 1.0 points(weather and time, police officers and their signal to stop) \\
- Key information 3 in the output is not mentioned in reference, deduction of -0.25 points. \\
No scores for:  \\
- Key information 3, 4, 5, 8, and 9. \\
% - Road Environment: Urban \\
% - Lane Options: Left Lane, Own Lane, Right Lane \\
% - Ego Lane Position: Middle Lane \\
% - Cannot change to the right lane as it's an merging lane and currently separated \\
% - Vehicles queuing in the left lane \\
Total score = (1.0 + 1.0 + 1.0 + 1.0 - 0.25) / 8 = 0.46875. \\
\bottomrule
\caption{Example of Alternative Action Sequences}
\label{tab:description}
\end{tabular}
\end{table*}
% \subsubsection{Scene Description Evaluation Example}
% \begin{minipage}{15em}
% - Case 1
% Output Description: 
% "There is a vehicle driving in the distance in front of you, there are traffic police on the left and right, and the traffic police signal to stop."
% Reference Description: 
% "You are driving on overhead road, the navigation information telling you to go straight through this road. There are currently ego lane and left lane ahead. The right lane is an merging lane and currently separated, so you cannot change lanes to the right.  There is police officers ahead inspecting passing vehicles. The police officer in front of your lane is signaling you to stop for inspection. There are also vehicles queuing in the left lane. Based on the current driving scenario, provide subsequent reasonable driving decisions."
% Prompt:
% {'role': 'system', 'content': 'You are a smart and logical evaluator with good knowledge of correct driving style, you will try your best to give reasonable and logical evaluation result.'}
% {'role': 'user', 'content': 'Given two driving scenario descriptions, one is reference descriptions, one is output descriptions from a model, please extract key information the reference description contains and use it as comparison standards to compare how close the output descriptions is to the reference descriptions also consider each information\'s completeness. Key information extracted can be classified into structured information and event specific information. Structured information are general driving scenario which includes road scenarios and weather scenarios, navigation information which describes the navigation or goal direction of the ego vehicle, lane ahead information which describe possible lane options ahead, and traffic control descriptions which includes traffic lights status and which lane the ego vehicle is driving on. Event specific information describe key event related to ego vehicle\'s driving decisions, they is usually given in the format of key object + verb/adj + influence to ego vehicle. An example of event specific information is like this: a construction zone is blocking the ego lane and the right lane in front, so the car needs to go around to avoid it.
% The reference description: ###
% You are driving on overhead road, the navigation information telling you to go straight through this road. There are currently ego lane and left lane ahead. The right lane is an merging lane and currently separated, so you cannot change lanes to the right.  There is police officers ahead inspecting passing vehicles. The police officer in front of your lane is signaling you to stop for inspection. There are also vehicles queuing in the left lane. Based on the current driving scenario, provide subsequent reasonable driving decisions.
% ###
% The output description: ###
% There is a vehicle driving in the distance in front of you, there are traffic police on the left and right, and the traffic police signal to stop.
% ###
% Compare the two descriptions using extracted key information and output a similarities score on the scale from 0 to 1.0 and a explanation to describe the logic to calculate the similarity score.
% Each matched key information scores 1.0, and each partially matched key information score 0.5. Hallucination will also be punished, each key information exists in output but not in reference will score -0.25, the final score will be the total score divided by the number of key information extracted in the reference description. For example if total score is 1.5, and total number of key information in reference description is 3, then the final score is 1.5/3 = 0.5.
% Output response in the format of json with score and explanation as keys. Json should follow text marks ###. Example of the output format is ###{"score": 0.6, "explanation": "<logic to calculate the score>"}###'}
% Response:
% Reference description key information:
% 1. Driving on overhead road (structured - general driving scenario) 
% 2. Navigation information is to go straight (structured - navigation information)
% 3. Ego lane and left lane available ahead (structured - lane ahead information)
% 4. Cannot change to the right lane as it\'s an merging lane and currently separated (structured - lane ahead information)
% 5. Police officers ahead inspecting vehicles (event specific information)
% 6. The police officer in front of ego vehicle signalling to stop (event specific information)
% 7. Vehicles queuing in the left lane (event specific information)
% Output description key information:
% 1. Vehicle driving in the distance in front of driver
% 2. Traffic police on the left and right
% 3. Traffic police signal to stop
% By comparing the output to the reference:
% - Key information 5 is matched, 1.0 points ("traffic police" close enough to "police officer" in meaning);
% - Key information 6 is matched, 1.0 points (both mention the police signal to stop);
% - Key information 1 in the output is not mentioned in reference, deduction of -0.25 points.
% No scores for: 
% - Driving on overhead road
% - Navigation information is to go straight
% - Ego lane and left lane available ahead
% - Cannot change to the right lane as it's an merging lane and currently separated
% - Vehicles queuing in the left lane
% Total score = (1.0 + 1.0 - 0.25) / 7 = 0.25.
% ###{"score": 0.25, "explanation": "Two key pieces of information (police officers and their signal to stop) from reference description were matched in the output and one key piece of information mentioned in the output description does not exist in the reference, which incurs a penalty."}###'
% Score: 0.25
% Explanation:"Two key pieces of information (police officers and their signal to stop) from reference description were matched in the output and one key piece of information mentioned in the output description does not exist in the reference, which incurs a penalty."
% \end{minipage}
% \begin{minipage}{15em}
% - Case 2
% Output Description:
% "The car is stopping at the intersection. There is a road ahead, pedestrians on the road are passing, and there is a police office directing the traffic. And there is a U-turn icon on the ground."
% Reference Description:
% "You are approaching an intersection. The navigation information is telling you to turn left in the intersection. There is some traffic on the left side of the intersection. You are in the left most lane and the left turn traffic light is green while going straight trafffic light is red. There are a bunch of pedestrians walking across the crosswalk in front of your car"
% Prompt:
% {'role': 'system', 'content': 'You are a smart and logical evaluator with good knowledge of correct driving style, you will try your best to give reasonable and logical evaluation result.'}
% {'role': 'user', 'content': 'Given two driving scenario descriptions, one is reference descriptions, one is output descriptions from a model, please extract key information the reference description contains and use it as comparison standards to compare how close the output descriptions is to the reference descriptions also consider each information's completeness. Key information extracted can be classified into structured information and event specific information. Structured information are general driving scenario which includes road scenarios and weather scenarios, navigation information which describes the navigation or goal direction of the ego vehicle, lane ahead information which describe possible lane options ahead, and traffic control descriptions which includes traffic lights status and which lane the ego vehicle is driving on. Event specific information describe key event related to ego vehicle's driving decisions, they is usually given in the format of key object + verb/adj + influence to ego vehicle. An example of event specific information is like this: a construction zone is blocking the ego lane and the right lane in front, so the car needs to go around to avoid it.
% The reference description: ###
% You are approaching an intersection. The navigation information is telling you to turn left in the intersection. There is some traffic on the left side of the intersection. You are in the left most lane and the left turn traffic light is green while going straight trafffic light is red. There are a bunch of pedestrians walking across the crosswalk in front of your car
% ###
% The output description: ###
% The car is stopping at the intersection. There is a road ahead, pedestrians on the road are passing, and there is a police office directing the traffic. And there is a U-turn icon on the ground
% ###
% Compare the two descriptions using extracted key information and output a similarities score on the scale from 0 to 1.0 and a explanation to describe the logic to calculate the similarity score.
% Each matched key information scores 1.0, and each partially matched key information score 0.5. Hallucination will also be punished, each key information exists in output but not in reference will score -0.25, the final score will be the total score divided by the number of key information extracted in the reference description. For example if total score is 1.5, and total number of key information in reference description is 3, then the final score is 1.5/3 = 0.5.
% Output response in the format of json with score and explanation as keys. Json should follow text marks ###. Example of the output format is ###{"score": 0.6, "explanation": "<logic to calculate the score>"}###'}
% Response:
% 'To start, let us identify the structured information and events specific information from the reference:
% - Structured Information:
% 1. Road scenario: intersection
% 2. Navigation information: turn left in the intersection
% 3. Lane ahead information: left most lane
% 4. Traffic control descriptions: left turn traffic light is green, going straight trafffic light is red
% - Event Specific Information:
% 1. Bunch of pedestrians walking across the crosswalk in front
% 2. Traffic on the left side of the intersection
% Given this, let\'s now compare the two descriptions:
% - Structured Information:
% 1. Intersection (match) - Score 1.0
% 2. U-turn icon on the ground (mismatch for left turn direction) - Score 0.0
% 3. Not specified which lane the car is on (mismatch) - Score 0.0
% 4. Traffic control by police officer (not mentioned in reference, hallucination) - Score -0.25
% - Event Specific Information:
% 1. Pedestrians passing the road (match) - Score 1.0
% 2. Not mention of traffic on the left side (mismatch) - Score 0.0
% Given that, the total score is 1.0 (intersection) + 0.0 (direction) + 0.0 (lane) - 0.25 (traffic control by police officer) + 1.0 (pedestrians) + 0.0 (traffic on left side) = 1.75
% As there were 6 pieces of key information in the reference that was evaluated against, the final similarity score is 1.75 / 6 = 0.29 (rounded off to the nearest hundredths)
% So the output will be:
% ###{"score": 0.29, "explanation": "The key information relevant to the intersection and pedestrians crossing were well captured. The direction of the navigation differed (U-turn vs. left turn), the lane of the vehicle was not specified and there was a hallucination related to a police officer controlling traffic. The traffic on the left side of the intersection was not mentioned which further reduces the similarity score."}###'
% Score: 
% 0.29
% Explanation:
% "The key information relevant to the intersection and pedestrians crossing were well captured. The direction of the navigation differed (U-turn vs. left turn), the lane of the vehicle was not specified and there was a hallucination related to a police officer controlling traffic. The traffic on the left side of the intersection was not mentioned which further reduces the similarity score."
% \end{minipage}

\subsection{Driving Decision Evaluation}
% In terms of evaluating driving decisions, it's vital to accurately and consistently assess the correct driving decisions, which can be expressed in various textual forms. To this end, we have introduced a predefined set of driving decision options, termed 'meta actions', and instructed the model to articulate its driving decisions as a sequence of these meta-actions. 

The evaluation process for the meta action sequence must account for both the quantity and the sequential arrangement of the matched meta actions. We use dynamic programming to compare the model's output and the established ground truth. 




% \includegraphics[width=0.99 \columnwidth]{imgs/ActionMap.png}
% The ground truth for each driving clip is manually annotated based on the actual driving action and trajectory, resulting in a unique sequence of meta-actions. 
% The meta-actions are designed to encompass all possible driving decisions, which can be distilled into a sequence of these actions. Furthermore, these meta-actions are structured to be readily extractable from vehicle trajectory data, with or without map information. They are categorized into three primary classes:
% \begin{enumerate}
%     \item Speed Control Actions: Primarily indicative of longitudinal control, these actions can be discerned from acceleration and braking signals within the vehicle data.
%     \item Turning Actions: These actions, relevant in the context of intersections, can be deduced from steering wheel signals.
%     \item Lane Control Actions: Encompassing lane selection decisions, these actions are derived from a combination of steering wheel signals and either map or perception data.
% \end{enumerate}

The dynamic programming approach employed in our study for evaluating the action sequences output by the model, in comparison to the reference sequences, bears resemblance to the method utilized in identifying the longest common subsequence, albeit with certain supplementary considerations. The first consideration acknowledges the unequal weighting of different meta-actions. For instance, certain meta-actions such as ``\textit{Slow Down}'', ``\textit{Wait}'', and ``\textit{Go Straight Slowly}'' are indicative of a conservative approach to driving decisions. The inclusion or exclusion of these actions from a meta-action sequence does not fundamentally alter the semantic essence of the driving decisions. Consequently, these are designated as ``conservative actions”, and a reduced penalty is imposed when these actions do not align in matching sequences.

The second consideration addresses the potential semantic equivalency among varying meta-action sequences. For example, the sequences ``\textit{Change Lane to the Left -> Speed Up -> Go Straight At a Constant Speed -> Change Lane to the Right}'' and ``\textit{Change Lane to the Left -> Speed Up Rapidly -> Go Straight At a Constant Speed -> Change Lane to the Right}'' might both represent valid approaches to overtaking a slow-speed vehicle ahead. 
% Each driving clip is manually annotated with a singular, definitive sequence of ground truth decisions and corresponding meta-actions. The Large Language Model (LLM) is then tasked with generating possible variations of this ground truth meta-action sequence that are semantically congruent.  
Recognizing that different meta-action sequences might convey semantically similar meanings, we first use the GPT-4 to generate variant sequences that are semantically akin, in addition to the unique ground truth meta-action sequence, as shown in Table~\ref{tab:alternative-actions}. In the subsequent sequence matching phase of the evaluation, all these variations, together with the manually annotated sequence, are taken into consideration. The highest-scoring match is then adopted as the definitive score for the final decision evaluation.


\begin{table*}[]
\centering
\begin{tabular}{p{\textwidth}}
\toprule
\textbf{Prompt:} \\

Given a predefined set of action tokens and a sequence of reference driving actions, find all alternative sequence of actions has similar meaning but choose slightly different actions tokens from the predefined action tokens. \\
Predefined action tokens: [Speed up, Slow down, Speed up rapidly, Slow down rapidly, Go straight slowly, Go straight at a constant speed, Turn left, Turn right, Change lane to the left, Change lane to the right, Shift slightly to the left, Shift slightly to the right, Stop, Wait, Turn around, Reverse]. \\
For example, if the reference driving action sequence is: Slow down -> Shift slightly to the right -> Go straight at a constant speed, alternative action sequences with similar meanings could be: \\
1. Slow down -> Change lane to the right -> Go straight at a constant speed; \\
2. Slow down rapidly -> Shift slightly to the right -> Go straight at a constant speed; \\
3. Slow down -> Change lane to the right -> Go straight slowly;  \\
4. Slow down -> Shift slightly to the right -> Go straight slowly. \\
Now the reference action sequence is: Slow down -> Shift slightly to the right -> Go straight at a constant speed. What are the alternative action sequences? \\

\midrule
\textbf{Response:} \\
Given the reference sequence: "Slow down -> Shift slightly to the right -> Go straight at a constant speed." Alternative action sequences with similar meanings based on the provided action tokens are: 
1. Slow down -> Change lane to the right -> Go straight at a constant speed. \\
2. Slow down rapidly -> Shift slightly to the right -> Go straight at a constant speed. \\
3. Slow down -> Change lane to the right -> Go straight slowly. \\
4. Slow down -> Shift slightly to the right -> Go straight slowly. You've provided this example in your question. \\
Based on the tokens and the context, these are indeed appropriate alternative sequences. \\
\bottomrule
\end{tabular}

\caption{Example of Alternative Action Sequences}
\label{tab:alternative-actions}
\end{table*}


The state of dynamic programming is saved in a 2D matrix, wherein each row corresponds to a meta action in the ground truth action sequence, and each column corresponds to a meta action in the model output action sequence. The dynamic programming initiates recursive calculations beginning from the first action of both sequences. Each element of the 2D matrix encompasses the optimal total score at the current matching position, as well as the preceding matching condition that yielded this optimal match. Our matching dynamic programming algorithm comprises three transition equations, corresponding respectively to three cases: missing match, redundant match, and successful match. The transformation equations for these cases are as follows:
\[S_{missing} = S_{r-1, c} - P_{missing}\]
\[S_{redundant} = S_{r, c-1} - P_{redundant}\]
\[S_{matching} = S_{r-1, c-1} + S_{successful}\]
\[S_{r,c} = max(S_{missing}, S_{redundant}, S_{matching})\]
In this framework, the $P_{missing}$ and the $P_{redundant}$ are quantified as half of $S_{successful}$ in instances where the action deemed missing or redundant is classified as a conservative action. Conversely, in scenarios where the action is not conservative, both penalties are assigned the same magnitude. This approach stems from the rationale that the omission of a key meta-action or the erroneous introduction of a non-existent key meta-action similarly impairs the efficacy of the resultant driving decision output.
